Choose Your QA Model Wisely: A Systematic Study of Generative and Extractive Readers for Question Answering

While both extractive and generative readers have been successfully applied to the Question Answering (QA) task, little attention has been paid toward the systematic comparison of them. Characterizing the strengths and weaknesses of the two readers is crucial not only for making a more informed reader selection in practice but also for developing a deeper understanding to foster further research on improving readers in a principled manner. Motivated by this goal, we make the first attempt to systematically study the comparison of extractive and generative readers for question answering. To be aligned with the state-of-the-art, we explore nine transformer-based large pre-trained language models (PrLMs) as backbone architectures. Furthermore, we organize our findings under two main categories: (1) keeping the architecture invariant, and (2) varying the underlying PrLMs. Among several interesting findings, it is important to highlight that (1) the generative readers perform better in long context QA, (2) the extractive readers perform better in short context while also showing better out-of-domain generalization, and (3) the encoder of encoder-decoder PrLMs (e.g., T5) turns out to be a strong extractive reader and outperforms the standard choice of encoder-only PrLMs (e.g., RoBERTa). We also study the effect of multi-task learning on the two types of readers varying the underlying PrLMs and perform qualitative and quantitative diagnosis to provide further insights into future directions in modeling better readers.

==> constrained_generation.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccc|cccccc}
\toprule
 \multirow{2}{*}{Generation Method} & \multicolumn{6}{c}{IID Datasets} & \multicolumn{6}{|c}{OOD Datasets}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 \hline

Regular &  91.54& 71.4 & 80.76 & {\bf 85.83} & {\bf 78.98} & 78.26 & {\bf 51.98} & 49.51 & 69.21 & 61.66 & 85.42 & 63.02\\ 
 C-Con   & {\bf 91.57} & {\bf 71.44} & 80.76 & 85.82 & 78.96 & 78.26 & 51.78 & {\bf 49.7} & {\bf 69.29} & 61.66 & {\bf 85.56} & 63.02\\  
NT-Con  & 91.52 & 71.42 & 80.73 & 85.75 & 78.93 & {\bf 78.27} & 51.76 & 49.66 & 69.23 & 61.66 & 85.49 & 63.02\\
\midrule
\# Novel tokens &  21 & 8 & 28 & 33 & 9 & 18  & 5 & 10 & 3 & 4 & 9 &5\\ 
\bottomrule
\end{tabular}
}
}
\caption{Test Multi task T5-Gen with three different generation methods. Regular: the reader can choose one of the tokens from the entire vocabulary. \# Novel tokens:number of novel tokens predicted by regular generation.}
\label{tab:gen_testing}
\end{table*}

==> gen_testing.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccccc|cccccc}
\toprule

\multirow{2}{*}{Target} & \multirow{2}{*}{Inference Method} & \multicolumn{6}{c}{In-domain Datasets} & \multicolumn{6}{|c}{Out-domain Datasets}\\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
~& ~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 \hline
A-Target & Regular & 91.56 & 71.26 & {\bf 81.01} & {\bf 86.62} & {\bf 79.65} & 77.89 & 50.88 & 49.95 & 69.03 & {\bf 63.13} & {\bf 85.88} & {\bf 63.04}\\
A-Target & C-Con  & 91.32 & 71.25 & 80.76 & 86.6 & 78.72 & 77.89 & 50.81 & 50.27 & 68.99 & 63.08 & 85.33 & 62.86\\  
A-Target & NT-Con   & 90.69 & 71.22 & 80.57 & 86.47 & 78.11 & 77.87 & 50.79 & 49.63 & 69.0 & 63.11 & 85.12 & 62.31\\
\hline
 C-Target & Regular &  91.54& 71.4 & 80.76 & {\bf 85.83} & {\bf 78.98} & 78.26 & {\bf 51.98} & 49.51 & 69.21 & 61.66 & 85.42 & 63.02\\ 
C-Target & C-Con   & {\bf 91.57} & {\bf 71.44} & 80.76 & 85.82 & 78.96 & 78.26 & 51.78 & {\bf 49.7} & {\bf 69.29} & 61.66 & {\bf 85.56} & 63.02\\  
C-Target & NT-Con  & 91.52 & 71.42 & 80.73 & 85.75 & 78.93 & {\bf 78.27} & 51.76 & 49.66 & 69.23 & 61.66 & 85.49 & 63.02\\
\toprule
\end{tabular}
}
}
\caption{Generative model trained by multi-tasks and evaluated by F1 score on each datasets. Regular: the reader can choose one of the token from the entire vocabulary; C-Con: the reader can choose one of the token from the context tokens and the end token(</s>); NT-Con: the reader can choose one of the token from the the next token of current predicted tokens in the context and the end token.}
\label{tab:gen_inference_all}
\end{table*}

==> new_tables/apd_table_f1_1024.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cccccc|cccccc}
\toprule

\multirow{2}{*}{Model} & \multirow{2}{*}{\diagbox{Train}{Test}} & \multicolumn{6}{c}{In-domain Datasets} & \multicolumn{6}{|c}{Out-domain Datasets}\\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
~& ~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 \hline
     \toprule
    \multicolumn{3}{l}{\bf Single Task Learning}\\
    \bottomrule
\multirow{6}{*}{T5-Ext} 
 & SQuAD & 92.47 & 64.97 & 62.09 & 37.29 & 71.03 & 64.54 & 52.01 & 50.13 & 68.66 & 52.58 & 85.78 & 58.61 \\
 & NewsQA & 87.38 & 72.22 & 62.26 & 40.79 & 66.56 & 68.35 & 31.72 & 49.72 & 65.97 & 55.11 & 78.75 & 58.72 \\
 & TQA   & 74.97 & 50.12 & 70.43 & 60.06 & 57.29 & 58.09 & 40.09 & 38.55 & 65.95 & 52.13 & 81.01 & 52.64 \\
 & SQA   & 72.47 & 47.96 & 68.45 & 77.10 & 53.54 & 56.63 & 41.57 & 35.53 & 66.07 & 51.89 & 81.63 & 50.31 \\
 & HQA   & 86.88 & 62.22 & 61.57 & 45.61 & 80.69 & 66.35 & 47.43 & 45.10 & 68.27 & 51.19 & 84.89 & 55.96 \\
 & NQ  &  86.73 & 64.28 & 64.39 & 53.21 & 68.56 & 79.08 & 53.14 & 52.06 & 71.26 & 61.07 & 84.35 & 56.15 \\
 \hline
 \multirow{6}{*}{T5-Gen} & SQuAD & 90.75 & 60.54 & 68.98 & 24.16 & 68.57 & 57.17 & 43.31 & 48.89 & 65.96 & 46.72 & 84.94 & 60.07\\
 & NewsQA  & 85.75 & 71.64 & 69.21 & 42.95 & 63.61 & 62.94 & 25.37 & 45.97 & 62.80 & 53.84 & 77.37 & 60.83 \\
 & TQA  & 74.33 & 49.26 & 79.02 & 57.61 & 58.75 & 54.88 & 33.84 & 42.38 & 56.94 & 51.16 & 80.52 & 52.42 \\
 & SQA  & 70.62 & 44.67 & 77.46 & 86.09 & 57.19 & 52.93 & 35.32 & 35.33 & 59.76 & 53.45 & 79.54 & 48.86 \\
 & HQA   & 86.24 & 60.27 & 70.47 & 51.93 & 79.87 & 62.13 & 44.94 & 46.38 & 66.93 & 42.66 & 84.56 & 59.38 \\
 & NQ   & 85.46 & 61.79 & 71.48 & 57.58 & 67.71 & 76.72 & 48.08 & 45.85 & 67.36 & 60.42 & 84.06 & 58.09 \\
 \hline
 \multirow{6}{*}{ELECTRA} 
 & SQuAD & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\  
 & NewsQA   & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\
 & TQA  & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\
 & SQA  & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 & HQA  & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\
 & NQ   & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\
 \hline
 \multirow{6}{*}{Roberta-Ext} 
 & SQuAD & 92.64 & 54.76 & 65.90 & 45.76 & 71.35 & 59.43 & 52.51 & 47.13 & 64.47 & 52.31 & 86.69 & 55.75 \\
 & NewsQA & 86.50 & 59.95 & 63.01 & 48.02 & 66.99 & 67.29 & 33.52 & 47.26 & 60.05 & 45.10 & 78.08 & 54.27 \\
 & TQA   & 73.63 & 41.05 & 72.97 & 51.16 & 62.44 & 55.76 & 44.40 & 39.27 & 54.92 & 42.72 & 82.32 & 49.89 \\
 & SQA   & 53.59 & 29.57 & 70.35 & 81.62 & 42.03 & 47.06 & 23.04 & 23.70 & 54.18 & 39.69 & 71.13 & 36.06 \\
 & HQA   & 85.10 & 50.55 & 65.06 & 44.31 & 81.21 & 63.88 & 51.74 & 36.86 & 62.44 & 37.49 & 85.07 & 54.02 \\
 & NQ  &  85.25 & 49.49 & 64.48 & 57.23 & 67.47 & 78.95 & 55.88 & 47.72 & 63.77 & 44.67 & 84.10 & 50.00 \\
 \hline
 \multirow{6}{*}{BART-Ext} 
 & SQuAD & 92.51 & 53.70 & 62.64 & 41.85 & 67.69 & 60.82 & 54.73 & 47.64 & 66.15 & 46.18 & 86.15 & 54.39 \\
 & NewsQA & 86.15 & 58.68 & 62.29 & 46.98 & 64.09 & 66.00 & 31.91 & 45.52 & 60.70 & 44.82 & 78.72 & 54.09 \\
 & TQA   & 69.82 & 38.40 & 72.55 & 61.02 & 61.05 & 54.10 & 34.63 & 36.36 & 54.34 & 39.35 & 81.28 & 46.43 \\
 & SQA   & 57.26 & 32.09 & 69.35 & 80.94 & 41.82 & 45.62 & 28.54 & 25.18 & 51.50 & 41.09 & 70.98 & 38.88 \\
 & HQA   & 83.29 & 49.66 & 63.18 & 40.46 & 80.71 & 63.52 & 47.91 & 38.56 & 59.78 & 34.60 & 84.32 & 52.04 \\
 & NQ  & 83.86 & 50.35 & 64.06 & 56.34 & 62.53 & 78.63 & 52.41 & 44.25 & 65.59 & 45.93 & 84.43 & 49.44 \\
\toprule
\multicolumn{3}{l}{\bf Multi-Task Learning}\\
\bottomrule
 T5-Ext & Multi  & 92.84 & 73.15 & 70.86 & 77.30 & 81.88 & 79.77 & 59.10 & 54.01 & 71.13 & 64.63 & 86.53 & 61.21\\
 \hline
 T5-Gen (base) & Multi  & 91.41 & 71.27 & 79.65 & 86.21 & 79.70 & 77.10 & 51.20 & 49.66 & 68.72 & 63.02 & 85.84 & 62.94\\ 
 \hline 
 ELECTRA & Multi & SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC\\
  \hline
 RoBERTa & Multi & 93.41 & 59.56 & 72.23 & 80.98 & 82.37 & 79.55 & 64.47 & 51.81 & 69.15 & 53.68 & 86.31 & 56.06\\
  \hline
 BART & Multi & 93.07 & 58.67 & 71.47 & 80.66 & 82.14 & 79.32 & 60.40 & 51.32 & 67.48 & 53.34 & 86.75 & 56.79\\
 \bottomrule
\end{tabular}
}
}
\caption{Evaluation by F1 score.  TQA: TriviaQA; SQA:SearchQA; HQA:HotpotQA; NQ: NaturalQuestions; TbQA:TextbookQA; RE:RelationExtraction. {\bf Bold} values are the best performance in a column for single-task and multi-task learning. All models are trained with 512 and tested with 1024 maximum length.}
\label{tab:apd_table_f1_1024}
\end{table*}

==> new_tables/compare_T5Gen_A_C_in.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule

\multirow{2}{*}{Model} & \multirow{2}{*}{\diagbox{Train}{Test}} & \multicolumn{2}{c|}{SQuAD} & \multicolumn{2}{c|}{NewsQA} &\multicolumn{2}{c|}{TQA} &\multicolumn{2}{c|}{SQA} &\multicolumn{2}{c|}{HQA} &\multicolumn{2}{c|}{NQ} &\multicolumn{2}{c}{Avg.} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}\cmidrule(lr){15-16}
~& ~& A & C & A & C & A & C & A & C & A & C & A & C & A & C\\ 
 \hline
\multirow{7}{*}{T5-Gen} 
 & SQuAD & \textbf{85.46} & 85.24 & \textbf{61.79} & 61.56 & 71.48 & \textbf{71.63} & 57.58 & \textbf{57.89} & \textbf{67.71} & 67.54 & \textbf{76.72} & 76.50 & \textbf{70.12} & 70.06\\ 
 & NewsQA & 85.75 & \textbf{85.85} & \textbf{71.64} & 71.31 & \textbf{69.21} & 68.79 & 42.95 & \textbf{43.27} & 63.61 & \textbf{63.94} & 62.94 & \textbf{63.04} & 66.02 & \textbf{66.03}\\
 & TQA   & 74.33 & \textbf{74.59} & 49.26 & \textbf{49.55} & \textbf{79.02} & 78.62 & 57.61 & \textbf{58.52} & \textbf{58.75} & 57.81 & 54.88 & \textbf{55.57} & 62.31 & \textbf{62.44}\\ 
 & SQA   &\textbf{ 70.62} & 70.20 & 44.67 & \textbf{44.82} & \textbf{77.46} & 76.96 & \textbf{86.09} & 85.25 & \textbf{57.19} & 55.31 & 52.93 & \textbf{53.00} & \textbf{64.83} & 64.26\\ 
 & HQA   & \textbf{86.24} & 86.05 & 60.27 & \textbf{60.70} & \textbf{70.47} & 69.91 & 51.93 & \textbf{52.39} & \textbf{79.87} & 79.82 & 62.13 & \textbf{62.31} & 68.48 & \textbf{68.53}\\ 
 & NQ  & \textbf{85.46} & 85.24 & \textbf{61.79} & 61.56 & 71.48 & \textbf{71.63} & 57.58 & \textbf{57.89} & \textbf{67.71} & 67.54 & \textbf{76.72} & 76.50 & \textbf{70.12} & 70.06\\ 
 & Multi & 91.41 & 91.16 & 71.27 & 70.81 & 79.65 & 79.42 & 86.21 & 85.06 & 79.70 & 78.90 & 77.10 & 76.31 & 80.89 & 80.28\\ 
\bottomrule
\end{tabular}
}
}
\caption{Compare two T5 generative readers on in-domain datasets, A: using A-Target to train T5-Gen, C: using C-Target to train T5-Gen.}
\label{tab:apd_compare_T5Gen_A_C_in}
\end{table*}

==> new_tables/compare_T5Gen_A_C_out.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule

\multirow{2}{*}{Model} & \multirow{2}{*}{\diagbox{Train}{Test}} & \multicolumn{2}{c|}{SQuAD} & \multicolumn{2}{c|}{NewsQA} &\multicolumn{2}{c|}{TQA} &\multicolumn{2}{c|}{SQA} &\multicolumn{2}{c|}{HQA} &\multicolumn{2}{c|}{NQ} &\multicolumn{2}{c}{Avg.} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}\cmidrule(lr){15-16}
~& ~& A & C & A & C & A & C & A & C & A & C & A & C & A & C\\ 
 \hline
\multirow{7}{*}{T5-Ext} 
 & SQuAD & 43.31 & 42.36 & 48.89 & 49.01 & 65.96 & 67.26 & 46.72 & 47.73 & 84.94 & 84.67 & 60.07 & 61.03 & 58.31 & 58.68\\ 
 & NewsQA & 25.37 & 25.33 & 45.97 & 46.42 & 62.80 & 61.90 & 53.84 & 53.05 & 77.37 & 77.48 & 60.83 & 60.67 & 54.36 & 54.14\\
 & TQA & 33.84 & 34.42 & 42.38 & 42.41 & 56.94 & 55.27 & 51.16 & 50.25 & 80.52 & 80.72 & 52.42 & 52.50 & 52.88 & 52.59\\ 
 & SQA & 35.32 & 34.46 & 35.33 & 36.23 & 59.76 & 55.39 & 53.45 & 51.37 & 79.54 & 77.78 & 48.86 & 49.07 & 52.04 & 50.72\\ 
 & HQA   & 44.94 & 44.46 & 46.38 & 45.32 & 66.93 & 65.61 & 42.66 & 43.51 & 84.56 & 84.54 & 59.38 & 58.32 & 57.48 & 56.96\\ 
 & NQ  & 48.08 & 48.20 & 45.85 & 45.25 & 67.36 & 67.08 & 60.42 & 60.56 & 84.06 & 83.47 & 58.09 & 57.96 & 60.64 & 60.42\\ 
 & Multi & 51.20 & 49.72 & 49.66 & 50.05 & 68.72 & 69.63 & 63.02 & 62.15 & 85.84 & 86.16 & 62.94 & 62.78 & 63.56 & 63.41\\ 
\bottomrule
\end{tabular}
}
}
\caption{Compare two T5 generative readers on out-of-domain datasets, A: using A-Target to train T5-Gen, C: using C-Target to train T5-Gen.}
\label{tab:apd_compare_T5Gen_A_C_in}
\end{table*}

==> new_tables/gen_method.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccc|cccccc}
\toprule
 \multirow{2}{*}{Generation Method} & \multicolumn{6}{c}{IID Datasets} & \multicolumn{6}{|c}{OOD Datasets}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
\midrule
Regular &  91.41 & 71.29 & 80.01 & 86.46 & 79.70 & 78.09 & 51.20 & 49.66 & 68.72 & 62.90 & 85.84 & 63.76\\ 
C-Con   & 91.18 & 70.79 & 80.08 & 84.96 & 78.88 & 77.35 & 51.07 & 49.74 & 68.62 & 62.89 & 85.49 & 63.63\\  
NT-Con  & 90.45 & 71.19 & 79.55 & 86.24 & 78.15 & 77.93 & 51.14 & 49.43 & 68.45 & 62.75 & 85.26 & 62.76\\
\midrule
Regular &  88.63 & 68.91 & 74.91 & 82.52 & 80.53 & 75.78 & 55.20 & 50.04 & 63.78 & 54.81 & 80.94 & 58.47\\ 
C-Con   & 72.91 & 47.47 & 44.38 & 63.69 & 58.68 & 62.33 & 37.83 & 35.51 & 44.33 & 37.64 & 64.80 & 38.01\\  
NT-Con  & 65.65 & 35.25 & 39.51 & 54.66 & 49.21 & 54.84 & 33.20 & 29.18 & 36.96 & 31.74 & 61.99 & 28.89\\
\midrule
\# Novel tokens &  21 & 8 & 28 & 33 & 9 & 18  & 5 & 10 & 3 & 4 & 9 &5\\ 
\bottomrule
\end{tabular}
}
}
\caption{Test Multi task T5-Gen with three different generation methods. Regular: the reader can choose one of the tokens from the entire vocabulary. \# Novel tokens:number of novel tokens predicted by regular generation.}
\label{tab:gen_method}
\end{table*}

==> new_tables/two_barts.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
Model & SQuAD & TQA & NQ \\
\toprule
BART(ED)-Ext & 92.51 & 72.55 & 78.63 \\ 
BART(ED)-Gen & 78.75 & 67.81 & 56.58 \\ 
\bottomrule
\end{tabular}
}
}
\caption{Comparison between BART extractive model (Ext-BART) and BART generative model (Gen-BART) using F1 metric. ED: both encoder and decoder. Inference Maximum length of 512.}
\label{tab:two_barts}
\end{table}

\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
Model & SQuAD & TQA & NQ \\
\toprule
T5(ED)-Ext & 90.57 & 66.86 & 76.69 \\ 
T5(ED)-Gen & 90.63 & 73.45 & 75.10 \\ 
\bottomrule
\end{tabular}
}
}
\caption{Comparison between T5(ED) generative and T5(ED) extractive models using F1 metric. ED: both encoder and decoder. Inference Maximum length of 512.}
\label{tab:two_barts}
\end{table}

==> novel_example.tex <==
\begin{table}[t]
    \centering 
    \small
\resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.3\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}@{}}
        \toprule
        \textbf{Question} & \textbf{Answer} & \textbf{Regular}& \textbf{C-Con} & \textbf{NT-Con}\\
        \toprule
        How fast is pharmacy informatics growing? &  quickly & rapidly & quickly & quickly\\
    \midrule
    What did Tesla work on in 1888? &  alternating current system & creating an alternating current system & an alternating current system & an alternating current system\\
    \midrule
    Money put in a collection plate at church & offering & coin & offering & offering\\
    \bottomrule
    \end{tabular}
    }
    \caption{Answers predicted by T5-Gen with different generation methods.}
    \label{tab:novel_example}
\end{table}


==> novel_example2.tex <==
\begin{table}[t]
    \centering 
    \small
\resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.1\linewidth}p{0.25\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}@{}}
        \toprule
         & \textbf{Context} & \textbf{Answer} & \textbf{Regular} & \textbf{C-Con} & \textbf{NT-Con}\\
        \toprule
        Text & ...(325 mi)... & 325 & 325 & (325 mi) & (325 mi)\\
        \\
        Tokens & $\_$(3, 25, $\_$mi, ) & $\_$3, 25 & $\_$3, 25  & $\_$(3, 25, $\_$mi, ) & $\_$(3, 25, $\_$mi, )\\
    \midrule
    Text & ...all-Gemini... & Gemini & Gemini & G mission & G mission \\ 
    \\
    Token & G, e, mini & $\_$Ge, mini & $\_$Ge, mini & $\_$G, $\_$mission & $\_$G, $\_$mission\\
    
    \bottomrule
    \end{tabular}
    }
    \caption{Tokens of answer and the predictions of T5-Gen using three generation methods.}
    \label{tab:novel_example2}
\end{table}


==> old_tables/main_table_em.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cccccc|cccccc}
\toprule

\multirow{2}{*}{Model} & \multirow{2}{*}{\diagbox{Train}{Test}} & \multicolumn{6}{c}{In-domain Datasets} & \multicolumn{6}{|c}{Out-domain Datasets}\\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
~& ~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 \hline
     \toprule
    \multicolumn{3}{l}{\bf Single Task Learning}\\
    \bottomrule
\multirow{6}{*}{T5-Ext} & SQuAD & 85.02 & 45.99 & 55.86 & 12.01 & 55.14 & 45.71 & 41.78 & 35.76 & 53.46 & 16.7 & 74.83 & 50.23\\
 & NewsQA   & 74.97 & 56.46 & 57.75 & 20.92 & 47.87 & 50.68 & 22.49 & 32.79 & 44.81 & 23.35 & 61.4 & 49.37\\
 & TQA   & 61.35 & 33.5 & 70.92 & 50.81 & 40.69 & 37.57 & 27.94 & 27.6 & 51.53 & 25.15 & 66.82 & 39.37\\
 & SQA   & 27.64 & 15.57 & 64.91 & 77.01 & 26.55 & 32.25 & 13.44 & 12.91 & 36.5 & 32.34 & 34.12 & 23.58\\
 & HQA   & 75.56 & 41.71 & 51.92 & 16.57 & 63.8 & 50.19 & 33.2 & 28.93 & 52.06 & 19.69 & 74.83 & 45.04\\
 & NQ   &70.58 & 40.81 & 56.56 & 34.4 & 48.6 & 68.61 & 33.0 & 31.6 & 52.13 & 39.39 & 69.27 & 42.5\\
 
 \hline
 \multirow{6}{*}{T5-Gen} & SQuAD & 83.62 & 43.61 & 61.27 & 21.58 & 52.5 & 46.34 & 33.8 & 35.16 & 52.13 & 37.99 & 73.68 & 49.7\\
 & NewsQA   & 73.94 & 55.03 & 60.51 & 35.58 & 45.21 & 48.27 & 18.83 & 33.98 & 40.43 & 40.85 & 59.06 & 49.77\\
 & TQA  & 65.52 & 34.9 & 75.74 & 55.74 & 41.98 & 40.36 & 25.68 & 30.56 & 45.81 & 43.65 & 69.37 & 42.84\\
 & SQA  & 63.65 & 33.43 & 73.42 & 80.84 & 43.57 & 39.81 & 24.82 & 28.34 & 47.67 & 46.11 & 68.89 & 43.5\\
 & HQA   & 77.65 & 42.55 & 62.61 & 43.0 & 63.79 & 49.6 & 34.66 & 32.94 & 52.53 & 34.8 & 74.93 & 47.63\\
 & NQ   & 73.53 & 42.55 & 62.67 & 48.63 & 50.33 & 65.02 & 38.26 & 35.01 & 46.81 & 50.77 & 70.93 & 47.5\\
 \hline
 \multirow{6}{*}{ELECTRA} & SQuAD &85.75 & 41.48 & 58.19 & 37.17 & 55.97 & 50.2 & 47.5 & 37.69 & 55.85 & 28.34 & 77.48 & 50.23\\ 
 & NewsQA   & 71.64 & 51.38 & 54.8 & 40.08 & 42.33 & 51.51 & 23.29 & 33.98 & 44.02 & 34.26 & 58.18 & 45.97\\
 
 & TQA  & 59.52 & 29.01 & 71.84 & 59.49 & 43.48 & 42.28 & 32.4 & 27.0 & 48.87 & 36.06 & 72.05 & 38.64\\
 & SQA  & 42.06 & 19.9 & 67.66 & 77.7 & 31.5 & 30.61 & 23.49 & 16.02 & 38.96 & 35.53 & 57.36 & 28.91\\
 & HQA   & 74.77 & 38.08 & 54.18 & 28.5 & 65.51 & 50.57 & 36.46 & 24.33 & 49.2 & 19.03 & 72.56 & 43.5\\
 & NQ   & 73.76 & 38.08 & 59.97 & 52.89 & 46.59 & 67.93 & 40.45 & 36.5 & 45.74 & 41.05 & 70.15 & 47.17\\
 \toprule
\multicolumn{3}{l}{\bf Multi-Task Learning}\\
\bottomrule
 T5-Ext & Multi  & 86.11 & 57.1 & 72.59 & 78.01 & 66.34 & 69.06 & 51.03 & 39.02 & 53.66 & 49.83 & 76.73 & 52.5\\
 \hline
 T5-Gen (base) & Multi  & 84.12 & 55.03 & 76.53 & 80.73 & 62.92 & 65.5 & 42.91 & 37.54 & 55.65 & 52.69 & 75.17 & 52.43\\
 T5-Gen (large) & Multi  & 86.74 & 56.91 & 79.85 & 83.52 & 67.43 & 67.47 & 54.22 & 42.43 & 60.04 & 59.08 & 77.1 & 57.69\\
 \hline
 ELECTRA & Multi  & 87.83 & 52.02 & 69.02 & 76.64 & 68.02 & 68.34 & 52.3 & 36.94 & 57.18 & 44.78 & 77.07 & 49.83\\
 \toprule
\end{tabular}
}
}
\caption{Evaluation by Exact Match(EM).  TQA: TriviaQA; SQA:SearchQA; HQA:HotpotQA; NQ: NaturalQuestions; TbQA:TextbookQA; RE:RelationExtraction}
\label{tab:main_table_em}
\end{table*}

==> old_tables/main_table_f1.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cccccc|cccccc}
\toprule

\multirow{2}{*}{Model} & \multirow{2}{*}{\diagbox{Train}{Test}} & \multicolumn{6}{c}{In-domain Datasets} & \multicolumn{6}{|c}{Out-domain Datasets}\\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
~& ~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & DROP & RACE & BioASQ & TbQA & RE & DuoRC \\ 
 \hline
     \toprule
    \multicolumn{3}{l}{\bf Single Task Learning}\\
    \bottomrule
\multirow{6}{*}{T5-Ext} & SQuAD & 92.27 & 64.36 & 65.55 & 17.76 & 71.42 & 60.7 & 53.47 & 49.05 & 68.71 & 23.7 & 85.56 & 60.89\\
 & NewsQA   & 86.89 & {\bf 72.76} & 67.99 & 27.57 & 67.65 & 65.62 & 31.79 & 48.64 & 66.76 & 33.68 & 79.47 & {\bf 62.37}\\

 & TQA   & 73.31 & 48.15 & 76.34 & 58.86 & 56.4 & 50.28 & 38.74 & 38.28 & 66.17 & 31.20 & 79.14 & 51.11\\
 & SQA   & 34.56 & 22.94 & 70.73 & 82.78 & 37.59 & 40.51 & 20.52 & 18.7 & 50.14 & 38.31 & 42.57 & 30.05\\
 & HQA   & 84.92 & 58.93 & 61.23 & 23.03 & 80.05 & 63.9 & 47.18 & 43.11 & 68.46 & 27.51 & 85.61 & 56.08\\
 & NQ  &  82.35 & 58.03 & 66.72 & 42.79 & 65.48 & {\bf 80.55} & 46.99 & 43.6 & {\bf 70.29} & 49.69 & 82.95 & 54.94\\
 \hline
 \multirow{6}{*}{T5-Gen} & SQuAD & 91.33 & 61.55 & 69.44 & 29.01 & 67.92 & 61.39 & 42.58 & 47.8 & 66.05 & 49.08 & 84.32 & 60.12 \\ 
 & NewsQA   & 86.51 & 71.6 & 69.74 & 43.07 & 64.59 & 63.53 & 26.01 & 47.83 & 61.11 & 54.38 & 77.77 &  61.56\\
 
 & TQA  & 76.84 & 51.41 & {\bf 80.1} & 63.36 & 58.64 & 56.21 & 34.05 & 42.48 & 57.94 & 52.43 & 81.91 & 54.32\\
 & SQA  & 74.63 & 48.09 & 78.13 & {\bf 85.93} & 58.65 & 54.59 & 31.68 & 39.67 & 59.31 & 54.21 & 79.93 & 53.35\\
 & HQA   & 86.07 & 59.96 & 70.61 & 52.21 & 79.88 & 63.59 & 43.73 & 45.1 & 66.16 & 42.6 & 85.34 & 58.24\\
 & NQ   & 85.4 & 62.15 & 71.68 & 58.01 & 67.41 & 78.17 & 48.09 & 46.99 & 66.33 & {\bf 60.74} & 83.84 & 59.17\\
 \hline
 \multirow{6}{*}{ELECTRA} & SQuAD & {\bf 93.08} & 58.31 & 66.49 & 46.16 & 71.75 & 66.36 & {\bf 58.74} & {\bf 50.86} & 70.21 & 39.89 & {\bf 87.36} & 59.83\\  
 & NewsQA   & 86.16 &65.21 & 63.88 & 49.72 & 61.83 & 67.96 & 32.05 & 49.08 & 64.87 & 48.74 & 78.3 & 57.26\\
 
 & TQA  & 70.69 & 42.46 & 76.51 & 67.79 & 60.61 & 57.7 & 42.19 & 36.66 & 62.27 & 44.06 & 83.28 & 49.01\\
 & SQA  & 51.54 & 28.59 & 72.12 & 82.93 & 43.6 & 41.11 & 30.72 & 21.76 & 53.28 & 42.67 & 70.66 & 35.77\\ 
 & HQA   & 84.97 & 53.72 & 61.94 & 36.9 & {\bf 81.21} & 64.93 & 48.55 & 37.39 & 65.2 & 26.55 & 84.66 & 53.19\\ 
 & NQ   & 85.75 & 55.12 & 67.88 & 62.14 & 64.06 & 79.67 & 53.7 & 50.69 & 67.76 & 50.94 & 83.83 & 56.54\\
 \hline
 \multirow{6}{*}{Roberta-Ext} 
 & SQuAD & 92.67 & 56.07 & 65.51 & 45.16 & 71.43 & 59.45 & 52.65 & 48.18 & 64.66 & 52.42 & 86.65 & 54.98\\
 & NewsQA & 86.45 & 59.32 & 63.17 & 47.58 & 66.69 & 66.94 & 33.39 & 45.87 & 60.66 & 46.17 & 78.08 & 54.77\\
 & TQA   & 73.64 & 42.45 & 72.52 & 50.96 & 62.34 & 55.64 & 44.48 & 39.22 & 54.88 & 41.39 & 82.31 & 49.81\\
 & SQA   & 53.56 & 29.43 & 70.05 & 81.34 & 41.89 & 46.96 & 22.53 & 23.65 & 53.67 & 38.51 & 71.13 & 37.39\\
 & HQA   & 85.15 & 51.35 & 64.57 & 44.02 & 80.88 & 63.83 & 51.17 & 37.25 & 61.94 & 37.07 & 85.07 & 54.43\\
 & NQ  &  85.28 & 49.73 & 63.60 & 56.26 & 66.89 & 78.82 & 55.02 & 46.36 & 63.62 & 44.99 & 84.1 & 50.81\\
 \hline
 \multirow{6}{*}{BART-Ext} 
 & SQuAD & 92.50 & 52.47 & 62.60 & 41.29 & 67.52 & 60.86 & 54.74 & 47.13 & 66.05 & 47.00 & 86.15 & 54.66\\
 & NewsQA & 86.16 & 58.81 & 61.62 & 46.37 & 63.79 & 65.88 & 31.2 & 45.30 & 60.51 & 44.2 & 78.72 & 54.37\\
 & TQA   & 69.88 & 38.6 & 72.11 & 60.97 & 61.00 & 54.17 & 34.62 & 35.84 & 53.87 & 38.84 & 81.28 & 47.18\\
 & SQA   & 57.29 & 31.95 & 69.14 & 80.33 & 41.65 & 45.76 & 28.48 & 24.35 & 51.15 & 40.88 & 70.98 & 39.7\\
 & HQA   & 83.27 & 49.3 & 63.25 & 40.34 & 80.30 & 63.14 & 48.47 & 38.1 & 59.90 & 34.4 & 84.32 & 52.39\\
 & NQ  & 83.85 & 50.68 & 63.96 & 55.99 & 62.19 & 78.57 & 51.92 & 43.68 & 65.19 & 45.2 & 84.43 & 50.26\\
\toprule
\multicolumn{3}{l}{\bf Multi-Task Learning}\\
\bottomrule
 T5-Ext & Multi   & 92.84 &  73.27 & 78.01 & 83.66 & 82.24 & {\bf 81.0} & 60.96 & 53.48 & 69.52 & 60.94 & 86.71 & 64.37\\
%  Ext & Multi (-NQA,-SQA) &92.31 & 56.34 & 70.96 & 63.73 & 81.8 & 78.13 & 56.28 & 50.6 & 69.54 & 48.13 & 85.86 & 55.04\\
 \hline
 T5-Gen (base) & Multi  & 91.54 & 71.4 & 80.76 &  85.83 & 78.98 & 78.26 & 51.98 & 49.51 & 69.21 &  61.66 & 85.42 & 63.02\\ 
 T5-Gen (large) & Multi & 93.54 & {\bf 73.44} & {\bf 84.08} & {\bf 88.38} & {\bf 82.88} & 80.58 & {\bf 63.63} & {\bf 55.87} & {\bf 72.33} & {\bf 68.76} & {\bf 87.33} & {\bf 68.09}\\
 \hline 
 ELECTRA & Multi & {\bf 93.92} & 65.33 & 73.63 & 81.94 & 83.36 & 79.98 & 61.77 & 52.71 & 71.86 & 54.8 & 87.18 & 59.76\\
%  Joint-base & Multi & 91.45$\downarrow$ & 71.41 & 80.79 & 85.62$\downarrow$ & 79.34$\uparrow$ & 78.14 & 51.11$\downarrow$ & 49.77$\uparrow$ & 69.68$\uparrow$ & 62.47$\uparrow$ & 85.66$\uparrow$ & 63.08\\
 \toprule
\end{tabular}
}
}
\caption{Evaluation by F1 score.  TQA: TriviaQA; SQA:SearchQA; HQA:HotpotQA; NQ: NaturalQuestions; TbQA:TextbookQA; RE:RelationExtraction. {\bf Bold} values are the best performance in a column for single-task and multi-task learning. }
\label{tab:main_table_f1}
\end{table*}

==> old_tables/single_task.tex <==
\begin{table*}[t]
\large
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|lllllll|lllllll}
\toprule

\multirow{2}{*}{Model} &  \multicolumn{7}{c}{In-domain Datasets} & \multicolumn{7}{|c}{Out-domain Datasets}\\
\cmidrule(lr){2-8} \cmidrule(lr){9-15}
~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & Avg. & DROP & RACE & BioASQ & TbQA & RE & DuoRC & Avg. \\ 
 \toprule
    \multicolumn{3}{l}{\bf Single Task Learning}\\
    \bottomrule
T5-Ext  & 92.27 & {\bf 72.76} & 76.34 & 82.78 &  80.05 & {\bf 80.55} & 80.79 & 53.47 &  49.05 & {\bf 70.29} & 49.69 & 85.61 & {\bf 62.37} & 61.75\\
T5-Gen  & 91.33  & 71.6 & {\bf 80.1} & {\bf 85.93} & 79.88 & 78.17 & {\bf 81.17} & 48.09 & 46.99 & 66.33 & {\bf 60.74} &  85.34 & 61.56 & 61.51\\
ELECTRA  & {\bf 93.08} & 65.21 & 76.51 & 82.93 & {\bf 81.21} & 79.69 & 79.77 & {\bf 58.74} & {\bf 50.86} & 70.21 & 50.94 & {\bf 87.36} & 59.83 & {\bf 62.99} \\
Roberta  & 92.67 & 59.32 & 72.52 & 81.34 & 80.88 & 78.82 & 77.59 & 55.02 & 48.18 & 64.66 & 52.42 & 86.65 & 54.98 & 60.32\\
Bart  & 92.50 & 58.81 & 72.11 & 80.33 & 80.30 & 78.57 & 77.10 & 54.74 & 47.13 & 66.05 & 47.00 & 86.15 & 54.66 & 59.29\\
\toprule
\multicolumn{3}{l}{\bf Multi-Task Learning}\\
\bottomrule
 T5-Ext &  92.84$_{\textcolor{blue}{+0.57}}$ & {\bf 73.27}$_{\textcolor{blue}{+0.51}}$ & 78.01$_{\textcolor{blue}{+1.67}}$ & 83.66$_{\textcolor{blue}{+0.88}}$ &  82.24$_{\textcolor{blue}{+2.19}}$ & {\bf 81.0}$_{\textcolor{blue}{+0.45}}$ & {\bf 81.84}$_{\textcolor{blue}{+1.05}}$ &  60.96$_{\textcolor{blue}{+7.49}}$ & {\bf 53.48}$_{\textcolor{blue}{+4.43}}$ &  69.52$_{\textcolor{red}{-0.77}}$ & 60.94$_{\textcolor{blue}{+11.25}}$ & 86.71$_{\textcolor{blue}{+1.1}}$ & {\bf 64.37}$_{\textcolor{blue}{+2.0}}$ &  {\bf 66.0}$_{\textcolor{blue}{+4.25}}$\\
%  Ext &92.31 & 56.34 & 70.96 & 63.73 & 81.8 & 78.13 & -& 56.28 & 50.6 & 69.54 & 48.13 & 85.86 & 55.04& -\\

 T5-Gen  & 91.54$_{\textcolor{blue}{+0.21}}$ & 71.4$_{\textcolor{red}{-0.2}}$ & {\bf 80.76}$_{\textcolor{blue}{+0.66}}$ & {\bf  85.83}$_{\textcolor{red}{-0.1}}$ & 78.98$_{\textcolor{red}{-0.9}}$ & 78.26$_{\textcolor{blue}{+0.09}}$& 81.13$_{\textcolor{red}{-0.04}}$ & 51.98$_{\textcolor{blue}{+3.9}}$ & 49.51$_{\textcolor{blue}{+2.5}}$ & 69.21$_{\textcolor{blue}{+2.9}}$ & {\bf 61.66}$_{\textcolor{blue}{+0.9}}$& 85.42$_{\textcolor{blue}{+0.1}}$ & 63.02$_{\textcolor{blue}{+1.5}}$& 63.47$_{\textcolor{blue}{+1.96}}$\\ 
ELECTRA & {\bf 93.92}$_{\textcolor{blue}{+0.84}}$ & 65.33$_{\textcolor{blue}{+0.12}}$ & 73.63$_{\textcolor{red}{-2.88}}$ & 81.94$_{\textcolor{red}{-0.99}}$ & {\bf 83.36}$_{\textcolor{blue}{+2.15}}$ & 79.98$_{\textcolor{blue}{+0.29}}$ & 79.69$_{\textcolor{red}{-0.08}}$ & {\bf 61.77}$_{\textcolor{blue}{+3.03}}$ & 52.71$_{\textcolor{blue}{+1.85}}$ & {\bf 71.86}$_{\textcolor{blue}{+1.65}}$ & 54.8$_{\textcolor{blue}{+3.86}}$ & {\bf 87.18}$_{\textcolor{red}{-0.18}}$ & 59.76$_{\textcolor{red}{-0.07}}$ & 64.68$_{\textcolor{blue}{+1.69}}$ \\
Roberta & 
93.36$_{\textcolor{blue}{+0.69}}$ & 60.15$_{\textcolor{blue}{+0.83}}$ & 71.40$_{\textcolor{red}{-1.12}}$  & 80.56$_{\textcolor{red}{-0.78}}$  & 82.21$_{\textcolor{blue}{+1.33}}$  & 79.50$_{\textcolor{blue}{+0.68}}$ & 77.86$_{\textcolor{blue}{+0.27}}$ & 64.79$_{\textcolor{blue}{+9.77}}$ & 51.49$_{\textcolor{blue}{+3.31}}$  & 68.69$_{\textcolor{blue}{+4.03}}$  & 53.68$_{\textcolor{blue}{+1.26}}$  & 86.31$_{\textcolor{red}{-0.34}}$  & 57.22$_{\textcolor{blue}{+2.24}}$  & 63.70$_{\textcolor{blue}{+3.38}}$ \\
Bart & 
93.06$_{\textcolor{blue}{+0.56}}$ & 58.72$_{\textcolor{red}{-0.09}}$ & 70.80$_{\textcolor{red}{-1.31}}$ & 80.11$_{\textcolor{red}{-0.22}}$ & 81.78$_{\textcolor{blue}{+1.48}}$ & 79.11$_{\textcolor{blue}{+0.54}}$ & 77.26$_{\textcolor{blue}{+0.16}}$ & 60.19$_{\textcolor{blue}{+5.45}}$ & 48.97$_{\textcolor{blue}{+1.84}}$ & 67.47$_{\textcolor{blue}{+1.42}}$ & 53.24$_{\textcolor{blue}{+6.24}}$ & 86.75$_{\textcolor{blue}{+0.60}}$ & 56.22$_{\textcolor{blue}{+1.56}}$ & 62.14$_{\textcolor{blue}{+2.85}}$\\
\hline
T5-Gen (large)  & 93.54 &  73.44 &  84.08 &  88.38 & 82.88  & 80.58 & 83.82 & 63.63 & 55.87 & 72.33 & 68.76 & 87.33 & 68.09 & 69.33\\
\hline 
\toprule 

\end{tabular}
}
}
\caption{Three readers trained by single and multi task learning and evaluated on in-domain and out-domain datasets by F1 Score.  TQA: TriviaQA; SQA:SearchQA; HQA:HotpotQA; NQ: NaturalQuestions; TbQA:TextbookQA; RE:RelationExtraction; Avg.: the Macro Average of in-domain/out-domain datasets. {\bf Bold} values are the best performance in a column for each block. }
\label{tab:single_task_f1}
\end{table*}

==> top5_f1.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccccc|ccccccc}
\toprule

\multirow{2}{*}{Model} &  \multicolumn{7}{c}{In-domain Datasets} & \multicolumn{7}{|c}{Out-domain Datasets}\\
\cmidrule(lr){2-8} \cmidrule(lr){9-15}
~& SQuAD & NewsQA & TQA & SQA & HQA & NQ & Avg. & DROP & RACE & BioASQ & TbQA & RE & DuoRC & Avg. \\ 
\toprule
\multicolumn{3}{l}{\bf Top1}\\
\bottomrule
 T5-Ext   & 92.84 & 73.27 & 78.01 & 83.66 & 82.24 &81.0  & 81.84 &  60.96 & 53.48 & 69.52 & 60.94 & 86.71 & 64.37 & 66.0\\
 T5-Gen  & 91.54 & 71.4 & 80.76 & 85.83 & 78.98 & 78.26 & 81.13 & 51.98 & 49.51 & 69.21 & 61.66 & 85.42 & 63.02 & 63.47\\ 
\toprule
    \multicolumn{3}{l}{\bf Top5}\\
\bottomrule
T5-Ext  & 97.31 & 86.9 & 88.72 & 91.14 & 93.88 & 91.93 & 91.65  & 82.03 & 68.36 & 84.51 & 74.2 & 93.83 & 75.18  &  79.68\\
T5-Gen  & 95.67 & 81.17 & 90.68 & 94.24 & 90.17 & 86.96 & 89.81 & 80.73 & 67.61 & 79.75 & 79.35 & 93.06 & 77.96  &  79.74\\
\toprule
    \multicolumn{3}{l}{\bf T5-Gen as Re-ranking Model}\\
\bottomrule
% Comb1 & 87.06 & 71.0 & 69.67 & 77.14 & 71.08 & 78.42 & 75.73  & 54.45 & 50.71 & 67.86 & 53.13 & 79.93 & 56.05  &  60.35\\
% Comb2 &  91.77 & 72.72 & 73.28 & 80.41 & 77.23 & 79.93 & 79.22 & 57.96 & 52.14 & 70.15 & 56.68 & 84.78 & 59.33 & 63.51\\
% Comb3 & 93.17 & 73.38 & 78.34 & 83.7 & 82.28 & 81.26 & 82.02 & 60.67 & 53.5 & 70.86 & 60.43 & 86.63 & 62.75 & 65.81 \\
Re-rank & 93.14 & 73.46 & 78.34 & 83.84 & 82.45 & 81.19  & 82.07  & 60.53 & 53.65 & 70.67 & 60.87 & 86.18 & 63.36 &  65.88\\
\toprule
    \multicolumn{3}{l}{\bf T5-Ext as Re-rankering Model}\\
\bottomrule
% Comb1 & 91.03 & 68.61 & 81.11 & 86.28 & 80.03  & 76.34 & 80.57 & 57.85 & 52.42 & 66.32 & 63.47 & 86.5 & 65.35 &  65.32\\
% Comb2 & 91.12 & 68.7 & 81.41 & 86.44 & 80.04 & 76.39 & 80.68 & 57.87 & 52.06 & 66.6 & 64.08 & 86.5 & 65.43 & 65.42\\
% Comb3 & 91.21 & 68.72 & 81.77 & 86.59 & 80.02 & 76.41 & 80.79  & 58.05 & 52.35 & 66.85 & 64.45 & 86.59 & 65.31 & 65.6\\
Re-rank & 91.03 & 68.61 & 81.11 & 86.28 & 80.03 & 76.34 & 80.57  & 57.85 & 52.42 & 66.32 & 63.47 & 86.5 & 65.35&  65.32\\
\bottomrule
\end{tabular}
}
}
\caption{Top5 Answers }
\label{tab:top5_answer}
\end{table*}
